Small Agents with Semantic Search: Efficient Multilingual Code Localization

Locating relevant files from natural-language requests is a core subtask for agents operating over code repositories. We investigate whether this task can be delegated to compact, specialized models to enable on-device search while reducing the token usage, latency, and inference cost of larger agents. We show that semantic search improves file localization, with gains in accuracy, cross-language transfer, and inference efficiency. To study this setting, we introduce a training framework for file-localization agents built around ColGREP, a local semantic search tool based on late-interaction retrieval models. Our recipe combines weighted supervised fine-tuning on teacher trajectories, assigning turn-level credit based on retrieval outcomes, with reinforcement learning on localization quality. We train three model families with fewer than two billion parameters to formulate search queries, inspect retrieved content, and identify relevant files. On localization tasks derived from SWE-bench Lite and Multi-SWE-bench Flash, ColGREP-equipped agents substantially improve over their base models and outperform corresponding GREP-based agents. In addition to improving localization accuracy, ColGREP reduces mean end-to-end trajectory latency by 44.1\% on CPU while using 29.1\% fewer tokens, and enables better generalization to programming languages unseen during fine-tuning. These results suggest that compact, tool-specialized localization agents can provide an efficient interface between natural-language requests and large codebases.

==> figures/assets/overview-icons.tex <==
% Small, original vector symbols. Colors are supplied by the caller.
\tikzset{
  pics/overview-student/.style={code={
    \draw[rounded corners=1pt] (-.49,-.3) rectangle (.49,.3);
    \draw (0,.3)--(0,.49); \fill (0,.52) circle (.055);
    \fill (-.19,.04) circle (.065); \fill (.19,.04) circle (.065);
    \draw (-.16,-.15)--(.16,-.15);
    \draw (-.61,-.13)--(-.61,.13) (.61,-.13)--(.61,.13);
  }},
  pics/overview-teacher/.style={code={
    \draw (-.64,.14)--(0,.42)--(.64,.14)--(0,-.13)--cycle;
    \draw (-.36,-.02)--(-.36,-.28) .. controls (0,-.47) .. (.36,-.28)--(.36,-.02);
    \draw (.6,.12)--(.6,-.36); \fill (.6,-.4) circle (.05);
  }},
  pics/overview-document/.style={code={
    \draw (-.38,-.48)--(-.38,.46)--(.12,.46)--(.39,.19)--(.39,-.48)--cycle;
    \draw (.12,.46)--(.12,.19)--(.39,.19);
    \draw (-.22,.04)--(.2,.04) (-.22,-.13)--(.2,-.13) (-.22,-.30)--(.1,-.30);
  }},
  pics/overview-files/.style={code={
    \draw (-.47,-.24)--(-.47,.45)--(.04,.45);
    \draw (-.24,-.46) rectangle (.44,.25);
    \draw (-.09,.06)--(.27,.06) (-.09,-.11)--(.27,-.11) (-.09,-.28)--(.15,-.28);
  }},
  pics/overview-ranking/.style={code={
    \foreach \y in {.32,0,-.32}{
      \fill (-.49,\y) circle (.065);
      \draw (-.20,\y)--(.51,\y);
    }
  }},
  pics/overview-trace/.style={code={
    \draw (-.44,.3)--(.35,.3)--(.35,-.3)--(-.44,-.3);
    \foreach \x/\y in {-.44/.3,.35/.3,.35/-.3,-.44/-.3}
      \fill[white] (\x,\y) circle (.10);
    \foreach \x/\y in {-.44/.3,.35/.3,.35/-.3,-.44/-.3}
      \draw (\x,\y) circle (.10);
  }},
  pics/overview-credit/.style={code={
    \foreach \x in {-.4,0,.4} \draw (\x,-.45)--(\x,.45);
    \foreach \x/\y in {-.4/.15,0/-.18,.4/.30}
      \filldraw[fill=white,rounded corners=.4pt] (\x-.12,\y-.07) rectangle (\x+.12,\y+.07);
  }},
  pics/overview-search/.style={code={
    \draw (-.12,.1) circle (.32);
    \draw (.12,-.14)--(.48,-.5);
  }},
  pics/overview-terminal/.style={code={
    \draw[rounded corners=1pt] (-.58,-.38) rectangle (.58,.38);
    \draw (-.36,.17)--(-.14,0)--(-.36,-.17) (.04,-.17)--(.33,-.17);
  }},
  pics/overview-request/.style={code={
    \draw[rounded corners=1pt] (-.54,-.2)--(-.54,.4)--(.54,.4)--(.54,-.2)
      --(-.1,-.2)--(-.37,-.44)--(-.37,-.2)--cycle;
    \foreach \x in {-.28,0,.28} \fill (\x,.09) circle (.045);
  }},
  pics/overview-learn/.style={code={
    \draw[-{Stealth[length=.85mm,width=.65mm]}] (.41,.12) arc[start angle=15,end angle=170,radius=.42];
    \draw[-{Stealth[length=.85mm,width=.65mm]}] (-.41,-.12) arc[start angle=195,end angle=350,radius=.42];
  }}
}%
\providecommand{\OverviewIcon}[2]{\raisebox{-.065cm}{%
  \tikz[x=.29cm,y=.29cm,draw=#1,fill=#1,line width=.55pt,
    line cap=round,line join=round,rounded corners=0pt]{%
    \path[use as bounding box] (-.7,-.6) rectangle (.7,.6);
    \pic {overview-#2};}}\hspace{.07cm}}%


==> figures/styles.tex <==
% Shared configuration. All diagrams are drawn at their final 13.6 cm width.
\RequirePackage{fix-cm}
\usetikzlibrary{arrows.meta,positioning,calc,fit,backgrounds}
\definecolor{figink}{HTML}{302A36}
\definecolor{figpurple}{HTML}{705D83}
\definecolor{figpale}{HTML}{F1EDF5}
\definecolor{figmid}{HTML}{D9CFE3}
\definecolor{figmuted}{HTML}{69636D}
\definecolor{figline}{HTML}{D8D3DC}
\definecolor{figgray}{HTML}{F7F6F8}
\definecolor{figteal}{HTML}{47776D}
\definecolor{figtealpale}{HTML}{EDF4F1}
\tikzset{
  paper figure/.style={x=1cm,y=1cm,font=\fontsize{8.5}{10.5}\selectfont,
    text=figink,line width=.6pt},
  fig box/.style={draw=figline,fill=white,rounded corners=2pt,
    align=center,inner sep=5pt,outer sep=0pt},
  fig accent/.style={fig box,draw=figpurple,fill=figpale},
  fig muted box/.style={fig box,fill=figgray},
  fig planned/.style={fig box,draw=figmuted,dash pattern=on 3pt off 2pt},
  fig arrow/.style={-{Stealth[length=1.7mm,width=1.25mm]},draw=figpurple,line width=.75pt},
  fig gray arrow/.style={fig arrow,draw=figmuted},
  fig planned arrow/.style={fig gray arrow,dash pattern=on 3pt off 2pt},
  fig label/.style={font=\fontsize{8}{9.5}\selectfont,text=figmuted,align=center},
  fig small/.style={font=\fontsize{7.5}{9}\selectfont,text=figmuted},
  fig heading/.style={font=\fontsize{9}{11}\selectfont\bfseries,text=figpurple,align=left},
  fig tile/.style={draw=figpurple,fill=figpale,rounded corners=1pt,
    minimum width=.52cm,minimum height=.48cm,inner sep=0pt,font=\bfseries},
  fig other tile/.style={fig tile,draw=figmuted,fill=white,dashed}
}

